Neural Compress-and-Forward for the Relay Channel

The relay channel, consisting of a source-destination pair and a relay, is a fundamental component of cooperative communications. While the capacity of a general relay channel remains unknown, various relaying strategies, including compress-and-forward (CF), have been proposed. For CF, given the correlated signals at the relay and destination, distributed compression techniques, such as Wyner-Ziv coding, can be harnessed to utilize the relay-to-destination link more efficiently. In light of the recent advancements in neural network-based distributed compression, we revisit the relay channel problem, where we integrate a learned one-shot Wyner--Ziv compressor into a primitive relay channel with a finite-capacity and orthogonal (or out-of-band) relay-to-destination link. The resulting neural CF scheme demonstrates that our task-oriented compressor recovers "binning" of the quantized indices at the relay, mimicking the optimal asymptotic CF strategy, although no structure exploiting the knowledge of source statistics was imposed into the design. We show that the proposed neural CF scheme, employing finite order modulation, operates closely to the capacity of a primitive relay channel that assumes a Gaussian codebook. Our learned compressor provides the first proof-of-concept work toward a practical neural CF relaying scheme.

==> EO_FC_SG_EE_Neural-Compress-and-Forward-for-the-Relay-Channel/common.tex <==
% Utility file


\usepackage{amsmath,amssymb,amsfonts,bbm,bm,mathrsfs}
\usepackage{color}
\usepackage{algorithmic}
\usepackage{graphicx}
\usepackage{textcomp}
\usepackage{xcolor}
% \usepackage{hyperref}
\usepackage{amsthm}

% \usepackage{flushend}

\usepackage[ruled,vlined,linesnumbered]{algorithm2e}

\usepackage[mode=tex]{standalone} % mode=image|tex, mode=build, buildmissing


\usepackage{tikz}
% \usepackage{tkz-graph}

\usepackage{chronosys}
\usepackage{xspace}
\usetikzlibrary{shapes,arrows,calc,positioning,fit,automata}
\usetikzlibrary{decorations.markings}
\usetikzlibrary{overlay-beamer-styles}
\usepackage{fontawesome}

\usepackage{pgfplots}
\usepackage{pgfplotstable}
\usepackage{filecontents}

\usepackage{caption,subcaption}

\usepackage{soul}


\newcommand{\Xcal}{\mathcal{X}}
\newcommand{\Pcal}{\mathcal{P}}
\newcommand{\Qcal}{\mathcal{Q}}
\newcommand{\Mcal}{\mathcal{M}}
\newcommand{\Gcal}{\mathcal{G}}
\newcommand{\Fcal}{\mathcal{F}}
\newcommand{\Phat}{\hat{P}}
\newcommand{\Xhat}{\hat{X}}
\newcommand{\xhat}{\hat{x}}
\newcommand{\Ptilde}{\tilde P}
\newcommand{\ptilde}{\tilde p}
\newcommand{\E}{\mathbb{E}}
\newcommand{\funF}{\mathrm{f}}
\newcommand{\funC}{\mathrm{c}}
\newcommand{\funQ}{\mathrm{q}}
\newcommand{\funG}{\mathrm{g}}
\newcommand{\funD}{\mathrm{d}}
\newcommand{\funID}{\mathrm{id}}
\newcommand{\classL}{\mathrm{L}}

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\sgn}{sgn}


\newcommand{\define}{\triangleq}
\newcommand{\eps}{\varepsilon}
\newcommand{\transpose}{\intercal}
\newcommand{\dmin}{d_{\mathrm{min}}}
\newcommand{\mat}[1]{\ensuremath{\mathbf{#1}}}
\newcommand{\vect}[1]{\ensuremath{\mathbf{#1}}}
\newcommand{\sign}[1]{\mathrm{sgn}\left(#1\right)}
\newcommand{\Norm}[1]{\left\lVert#1\right\rVert}
\newcommand{\norm}[1]{||#1||}

\newcommand{\Pilots}{\mat{\tilde{X}}}
\newcommand{\pilots}{\vect{\tilde{x}}}

\newcommand{\NoiseQuant}{\mat{\delta Q}}
\newcommand{\noiseQuant}{\vect{\delta q}}
\newcommand{\NoisePilots}{\mat{Z}}
\newcommand{\noisePilots}{\vect{z}}


\newcommand{\myBlue}{blue!80!black}
\newcommand{\myGreen}{green!60!black}
\newcommand{\myRed}{red!80!black}


\newcommand{\Ndata}{N_\text{data}}
\newcommand{\Nsc}{N_\text{sc}}
\newcommand{\Nse}{N_\text{se}}
\newcommand{\Nfft}{N_\text{FFT}}
\newcommand{\Ptx}{P_\text{TX}}
\newcommand{\EBW}{\text{EBW}}
\newcommand{\ER}{\text{ER}}
\newcommand{\SNR}{\text{SNR}}
\newcommand{\SER}{\text{SER}}
\newcommand{\PAPR}{\text{PAPR}}



\newcommand{\noteRed}[1]{{\color{red}#1}}
\newcommand{\noteBlue}[1]{{\color{blue}#1}}


\newcommand{\Enc}{\mathrm{e}_\theta}
\newcommand{\Demod}{\mathrm{p}_\phi}
\newcommand{\Demodprime}{\mathrm{p}_\xi}
\newcommand{\SWEnc}{}
\newcommand{\SWDec}{}
\newcommand{\EntEnc}{}
\newcommand{\EntDec}{}
\newcommand{\EntMod}{\mathrm{q}_\zeta}


\definecolor{NYUviolet}{HTML}{57068c} 	% official NYU violet
\definecolor{NYUlight}{HTML}{8900e1} 	% NYU light violet
\definecolor{NYUdark}{HTML}{330662} 	% NYU dark violet
\definecolor{NYUnight}{HTML}{220337} 	% NYU darker violet



\newcommand\blfootnote[1]{%
	\begingroup
	\renewcommand\thefootnote{}\footnote{#1}%
	\addtocounter{footnote}{-1}%
	\endgroup
}


\newcommand{\algorithmsize}{\small}

%\newcommand{\note}[1]{{\color{red}#1}}
\newcommand{\ToDo}[1]{{\color{red}\textbf{\underline{#1}}}}
\newcommand{\highlight}[1]{{\bfseries#1}}
% \newcommand{\review}[1]{{\color{blue}#1}}
\newcommand{\review}[1]{{#1}}

\tikzstyle{block}=[rectangle,draw,very thick,fill=white,align=center,font=\Large]
\tikzstyle{edge} = [draw,very thick,->,-triangle 45]
\tikzstyle{plateBlue} = [draw=\myBlue, shape=rectangle, rounded corners=0.5ex, ultra thick,
minimum width=3.1cm, text=\myBlue, text width=3.1cm, align=right, inner sep=10pt, inner ysep=10pt,append after command={node[font=\bf,text=\myBlue,above left= 3pt of \tikzlastnode.south east] {#1}}]

\tikzstyle{plateRed} = [draw=\myRed, shape=rectangle, rounded corners=0.5ex, ultra thick,
minimum width=3.1cm, text=\myRed, text width=3.1cm, align=right, inner sep=10pt, inner ysep=10pt,append after command={node[font=\bf\LARGE,text=\myRed,above= 3pt of \tikzlastnode.south] {#1}}]


\tikzstyle{plateGreen} = [draw=\myGreen, shape=rectangle, rounded corners=0.5ex, ultra thick,
minimum width=3.1cm, text=green!80!black, text width=3.1cm, align=right, inner sep=10pt, inner ysep=10pt,append after command={node[font=\bf\LARGE,text=\myGreen,above= 3pt of \tikzlastnode.south] {#1}}]


\tikzstyle{plate} = [draw, shape=rectangle, rounded corners=0.5ex, ultra thick,
minimum width=3.1cm,  text width=3.1cm, align=right, inner sep=10pt, inner ysep=10pt,append after command={node[font=\bf\Large,above left= 3pt of \tikzlastnode.south east] {#1}}]


\tikzstyle{plateSmall} = [draw, shape=rectangle, rounded corners=0.5ex, ultra thick,
minimum width=3.1cm,  text width=3.1cm, align=right, inner sep=10pt, inner ysep=10pt,append after command={node[font=\bf,above= 3pt of \tikzlastnode.south] {#1}}]

\tikzstyle{plateUp} = [draw, shape=rectangle, rounded corners=0.5ex, ultra thick,
minimum width=3.1cm,  text width=3.1cm, align=right, inner sep=10pt, inner ysep=10pt,append after command={node[font=\bf\Large,above= 3pt of \tikzlastnode.north] {#1}}]

\tikzstyle{plateUpEast} = [draw, shape=rectangle, rounded corners=0.5ex, ultra thick,
minimum width=3.1cm,  text width=3.1cm, align=right, inner sep=10pt, inner ysep=10pt,append after command={node[font=\bf\Large,above= 3pt of \tikzlastnode.north east, anchor=south east] {#1}}]

\tikzstyle{plateDown} = [draw, shape=rectangle, rounded corners=0.5ex, ultra thick,
minimum width=3.1cm,  text width=3.1cm, align=right, inner sep=10pt, inner ysep=10pt,append after command={node[font=\bf\Large,below= 3pt of \tikzlastnode.south] {#1}}]


\usepackage[prefix=]{xcolor-material}
\pgfmathdeclarerandomlist{material}{%
	{Red}{Blue}{Green}}
\tikzset{%
	half clip/.code={
		\clip (0, -256) rectangle (256, 256);
	},
	color/.code=\colorlet{fill color}{#1},
	color alias/.code args={#1 as #2}{\colorlet{#1}{#2}},
	colors alias/.style={color alias/.list/.expanded={#1}},
	execute/.code={#1},
	on left/.style={.. on left/.style={#1}},
	on right/.style={.. on right/.style={#1}},
	split/.style args={#1 and #2}{
		on left ={color alias=fill color as #1},
		on right={color alias=fill color as #2, half clip}
	}
}
\newcommand\reflect[2][]{%
	\begin{scope}[#1]\foreach \side in {-1, 1}{\begin{scope}
				\ifnum\side=-1 \tikzset{.. on left/.try}\else\tikzset{.. on right/.try}\fi
				\begin{scope}[xscale=\side]#2\end{scope}
\end{scope}}\end{scope}}

\tikzset{%
	cat/.pic={
		\tikzset{x=1.5cm/5,y=1.5cm/5,shift={(0,-1/3)}}
		\useasboundingbox (-1,-1) (1,2);
		\fill [BlueGrey900] (0,-2)
		.. controls ++(180:3) and ++(0:5/4) .. (-2,0)
		arc (270:90:1/5)
		.. controls ++(0:2) and ++(180:11/4) .. (0,-2+2/5);
		\foreach \i in {-1,1}
		\scoped[shift={(1/2*\i,9/4)}, rotate=45*\i]{
			\clip [overlay] (0, 5/9) ellipse [radius=8/9];
			\clip [overlay] (0,-5/9) ellipse [radius=8/9];
			\fill [BlueGrey900] ellipse [radius=1];
			\clip [overlay] (0, 7/9) ellipse [radius=10/11];
			\clip [overlay] (0,-7/9) ellipse [radius=10/11];
			\fill [Purple100] ellipse [radius=1];
		};
		\fill [BlueGrey900] ellipse [x radius=3/4, y radius=2];
		\fill [BlueGrey100] ellipse [x radius=1/3, y radius=1];
		\fill [BlueGrey900]
		(0,15/8) ellipse [x radius=1, y radius=5/6]
		(0, 8/6) ellipse [x radius=1/2, y radius=1/2]
		{[shift={(-1/2,-2)}, rotate= 10]  ellipse [x radius=1/3, y radius=5/4]}
		{[shift={( 1/2,-2)}, rotate=-10] ellipse [x radius=1/3, y radius=5/4]};
		\fill [BlueGrey500]
		(-1/9,11/8) ellipse [x radius=1/5, y radius=1/5]
		( 1/9,11/8) ellipse [x radius=1/5, y radius=1/5];
		\fill [Purple100]
		(0,12/8)     ellipse [x radius=1/10, y radius=1/5]
		(0,12/8+1/9) ellipse [x radius=1/5 , y radius=1/10];
		\foreach \i in {-1,1}
		\scoped[shift={(1/2*\i,2)}, rotate=35*\i]{
			\clip [overlay] (0, 1/7) ellipse [radius=2/7];
			\clip [overlay] (0,-1/7) ellipse [radius=2/7];
			\fill [Yellow50] ellipse [radius=1];
		};
		\scoped{
			\clip (-1,-2) rectangle ++(2,1);
			\fill [BlueGrey900] (0,-2) ellipse [radius=1/2];
			\fill [Grey100]
			(-1/2,-2) ellipse [x radius=1/3, y radius=1/4]
			( 1/2,-2) ellipse [x radius=1/3, y radius=1/4];
		};
		\foreach \i in {-1,1}
		\foreach \j in {-1,0,1}
		\fill [Grey100, shift={(0,11/8)}, xscale=\i, rotate=\j*15,
		shift=(0:1/2)]
		ellipse [x radius=1/3, y radius=1/64];
	},
dog/.pic={
	\begin{scope}[x=1.5cm/480,y=1.5cm/480]
		\useasboundingbox (-256, -256) (256, 256);
		\reflect[split=Brown400 and Brown500]{
			\fill [fill color] (0,-64) ellipse [x radius=160, y radius=144];
			\fill [fill color] (0, 32) ellipse [x radius=128, y radius=112];
			\fill [fill color] (32,96)
			.. controls ++( 75:128) and ++(105:128) .. ++(192,  0)
			.. controls ++(285: 96) and ++(285: 96) .. ++(-80,-32)
			.. controls ++(105: 64) and ++( 75: 32) .. cycle;
		}
		\reflect[split={Grey100 and Grey200}]{
			\clip (0,-64) ellipse [x radius=160, y radius=144];
			\fill [fill color](0,-224) 
			.. controls ++(  0:64) and ++(270:64) .. ++(96,64)
			.. controls ++( 90:64) and ++(270:64) .. ++(-96,192)
			.. controls ++(270:64) and ++( 90:64) .. ++(-96,-192)
			.. controls ++(270:64) and ++(180:64) .. cycle;
		}
		\reflect[split={Pink100 and Pink200}]{
			\fill [fill color](0,-192) ellipse [x radius=28, y radius=32];
		}
		\reflect[split={BlueGrey800 and BlueGrey900}]{
			\fill [fill color](0,-144) 
			.. controls ++(  0:20) and ++(315:20) .. ++( 40,64)
			.. controls ++(135:20) and ++( 45:20) .. ++(-80, 0)
			.. controls ++(225:20) and ++(180:20) .. cycle;
			\fill [BlueGrey900] (56, 0) circle [radius=20];
			\fill [fill color] (-8,-112)
			-- ++(16,0) -- ++(0,-32) arc (180:360:24)
			arc (180:0:8) arc (360:180:40);
		}
\end{scope}}
}

\tikzset{
	o/.style={
		shorten >=#1,
		decoration={
			markings,
			mark={
				at position 1
				with {
					\draw circle [radius=#1];
				}
			}
		},
		postaction=decorate
	},
	o/.default=2pt
}




%% FROM https://tex.stackexchange.com/questions/103849/telecommunications-symbols


\tikzset{naming/.style={align=center,font=\large}}
\tikzset{antenna/.style={insert path={-- coordinate (ant#1) ++(0,0.25) -- +(135:0.25) + (0,0) -- +(45:0.25)}}}
\tikzset{station/.style={naming,draw,shape=dart,shape border rotate=90, minimum width=15mm, minimum height=30mm,outer sep=0pt,inner sep=3pt}}
\tikzset{stationPoster/.style={naming,draw,shape=dart,shape border rotate=90, minimum width=20mm, minimum height=40mm,outer sep=0pt,inner sep=3pt}}
%\tikzset{mobile/.style={naming,draw,shape=rectangle,minimum width=15mm,minimum height=7.5mm, outer sep=0pt,inner sep=3pt}}
\tikzset{mobile/.style={naming,draw,shape=rectangle,minimum width=12mm,minimum height=6mm, outer sep=0pt,inner sep=3pt}}
\tikzset{radiation/.style={{decorate,decoration={expanding waves,angle=90,segment length=4pt}}}}




\newcommand{\MBS}[1]{%
\begin{tikzpicture}
\node[station] (base) {#1};


\draw[line join=bevel] (base.100) -- (base.80) -- (base.120) -- (base.60) -- (base.mid west) -- (base.mid east);
\draw[line join=bevel] (base.mid east) -- (base.120) -- (base.60) (base.60) -- (base.100);

% \draw[line join=bevel] (base.95) -- (base.310);
% \draw[line join=bevel] (base.105) -- (base.300);
% \draw[line join=bevel] (base.120) -- (base.270);
% \draw[line join=bevel] (base.180) -- (base.220);

% \draw[line join=bevel] (base.100) -- (base.80) -- (base.110) -- (base.70) -- (base.north west) -- (base.north east);
% \draw[line join=bevel] (base.100) -- (base.70) (base.110) -- (base.north east);

\draw[line cap=rect] ([xshift=-5mm,yshift=0mm]base.north -| base.right tail) [antenna=1];
\draw[line cap=rect] ([yshift=0mm]ant1 |- base.north) -- node[above,shape=rectangle,inner ysep=5]{\dots} ([xshift=5mm, yshift=0mm]base.north -| base.left tail) [antenna=2];

\end{tikzpicture}
}


\newcommand{\MBSposter}[1]{%
\begin{tikzpicture}
    \node[stationPoster] (base) {#1};
    
    \draw[line join=bevel] (base.100) -- (base.80) -- (base.120) -- (base.60) -- (base.mid west) -- (base.mid east);
    \draw[line join=bevel] (base.mid east) -- (base.120) -- (base.60) (base.60) -- (base.100);
    
    \draw[line cap=rect] ([xshift=-5mm,yshift=0mm]base.north -| base.right tail) [antenna=1];
    \draw[line cap=rect] ([yshift=0mm]ant1 |- base.north) -- node[above,shape=rectangle,inner ysep=5]{\scriptsize\dots} ([xshift=5mm, yshift=0mm]base.north -| base.left tail) [antenna=2];

\end{tikzpicture}
}
